Predicting Performance for Natural Language Processing Tasks

Given the complexity of combinations of tasks, languages, and domains in natural language processing (NLP) research, it is computationally prohibitive to exhaustively test newly proposed models on each possible experimental setting. In this work, we attempt to explore the possibility of gaining plausible judgments of how well an NLP model can perform under an experimental setting, without actually training or testing the model. To do so, we build regression models to predict the evaluation score of an NLP experiment given the experimental settings as input. Experimenting on 9 different NLP tasks, we find that our predictors can produce meaningful predictions over unseen languages and different modeling architectures, outperforming reasonable baselines as well as human experts. Going further, we outline how our predictor can be used to find a small subset of representative experiments that should be run in order to obtain plausible predictions for all other experimental settings.

==> sections/limitation.tex <==
% 1. for model comparisons, our models are usually very similar to each other, and the performance is similar to each other
% 2. for performance prediction, we fail in cases we didn't cover in our experiments

\gn{I would just put this in the conclusion. Also, maybe be a bit more positive in the wording here? I think the results are very interesting, so I don't think we need to dump on them too much.}

Though we try to verify the validity and effectiveness of our predictors in various ways, we are still faced with a number of limitations, and these limitations unfortunately impede some real applications on real scenarios. We list out these deficiencies and leave them as future work.

\paragraph{Homogeneous v.s. Heterogeneous} Though we collect a number of experiment records for each tasks, they are actually restricted in certain conditions. First of all, for example, as mentioned in \ref{sec:formulation}, we leave possible domain shift between training set and test set out. Second, our predictor may still not be able to generalize well to of some features, such as sentence length and subword vocabulary. For example, the average sentence length of wikimatrix is limited to 10-30 and it's set to a 5000 subword size for datasets. Therefore, we unsurprisingly find that the predictor provides nonsensical predictions for datasets that have a shorter average sentence length (e.g. 5), because it fails to capture the correlation between short sentence lengths and performance. To broadly expand the idea to real scenarios where there exists a drastic increase in complexity, ideally we could index all existing results for a certain task to build a more robust predictor.
\an{I think it would be very beneficial to add the Portuguese/Mapudungun example here}


\paragraph{Various Models} Though we do comparisons across models, the multi-model tasks we evaluate on do not really cover computationally intensive ones such as machine translation. Also, the model


==> tables/model.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccc} \toprule
%                       & Mean & RMSE@1 & RMSE@2 & RMSE@3 & RMSE@4 & RMSE@5 \\ \midrule
% CHARLES-SAARLAND-02-2 & 6.04   & 4.45   & 4.33   & 4.07   & {\bf 3.55}   & 4.21   \\
% OHIOSTATE-01-2        & {\bf 3.50}   & 4.73   & 4.54   & 4.55   & 4.58   & 4.59   \\
% CARNEGIEMELLON-02-2   & 7.47   & 8.16   & 7.60   & 7.33   & 7.34   & {\bf 7.18}   \\
% EDINBURGH-01-2        & 2.39   & {\bf 2.09}   & 2.19   & 2.16   & 2.28   & 2.22   \\
% Unknown               & 6.38   & 4.86   & 4.68   & 4.40   & 4.22   & {\bf 4.17}   \\
% CMU-01-2-DataAug      & {\bf 5.57}   & 6.42   & 6.16   & 6.04   & 5.79   &  5.74   \\ \midrule
% All                   & 5.23   & 5.12   & 4.92   & 4.76   & {\bf 4.62}   & 4.69  \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
         & RMSE@0 & RMSE@1 & RMSE@2 & RMSE@3 & RMSE@4 & RMSE@5 \\
\midrule
UDPipe   & 6.78   & 3.53   & 3.26   & 3.05   & 3.18   & {\bf 2.99}   \\
TurkuNLP & 6.70   & 3.47   & 3.20    & 3.00    & 3.14   & {\bf 2.97}   \\
ICS      & 7.05   & 4.44   & 4.22   & {\bf 4.04}   & 4.20    & 4.08   \\
Stanford & 7.48   & 5.69   & {\bf 5.59}   & 5.62   & 5.64   & 5.68   \\
NLP-Cube & 4.93   & 3.13   & 3.01   & {\bf 2.96}   & 3.07   & 3.04   \\
HIT-SCIR & 9.80   & 5.19   & 4.82   & 4.61   & 4.89   & {\bf 4.51}   \\
\midrule
average & \\
\bottomrule
\end{tabular}
\caption{RMSE scores from a predictor trained with experiment records of other models and n (1/2/3/4/5) random examples of the new model, denoted as RMSE@n. RMSE@0 denotes the mean value baseline. \mz{ show the delta, best system and worst system, averages for all systems} \gn{I would make this a figure.}\an{Actually, maybe a small line graph per system?, so that they don't overlap, and we can put them in a 2x3 or 2x4 grid, as below (with more beautiful graphs than I did).}}
\label{tab:model}
\end{table*}

==> tables/rep.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{llrr}
\toprule
Task    & Best / Worst                                & BS RMSE & RS RMSE  \\ \midrule
BLI     & eng-tha, fin-eng, eng-ell, por-eng & 10.560 & 25.34   \\
        & eng-deu, eng-por, eng-spa, eng-fra & 44.414 & -  \\ \midrule
MA        & br\_keb, lt\_hse, da\_ddt, bxr\_bdt, fr\_spoken & 6.236 & 22.245\\  
& sa\_ufal, tl\_trg, cs\_pud, bxr\_bdt, fo\_oft & 44.362 & - \\ \midrule
UD & hu\_szeged, hu\_szeged, id\_gsd, kk\_ktb, ug\_udt & 11.582 \\ 
& bxr\_bdt, gl\_ctg, bxr\_bdt, fr\_spoken, gl\_ctg \\ \midrule

TED-MT      & ita-eng, kat-eng, bos-eng, mkd-eng, urd-eng & 5.688  & 10.894 \\
        & spa-eng, por-eng, fra-eng, nld-eng, dan-eng & 23.498 & -    \\ \midrule
% TSF-MT   & dan-vie, eus-ben, bos-tur, nld-tha, bel-tur & 6.365    & 15.215 \\
        % & por-swe, por-kaz, por-spa, por-mon, por-glg & 23.576 & -    \\ \midrule
Wiki-MT & eng-ukr, heb-srp, ind-bos, ita-por, por-spa & 4.163    & 16.853 \\
        & eng-spa, por-eng, glg-spa, spa-eng, srp-bos & 26.672 & -  \\ \bottomrule
\end{tabular}
\caption{The beam search (BS RMSE) results for the 5 most representative datasets of multiple tasks with a beam size 100 and the random search (RS RMSE) results.}
\label{tab:rep}
\end{table*}

==> tables/unseen.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
Unseen & Wiki-MT & TSF-MT & TSF-PARSING & TSF-POS & TSF-EL & BLI \\ \midrule
Source    & 2.58    & 7.94   & 10.60       & 29.78   & 26.23  &  3.37   \\
Target    & 2.79    & 1.46   & 8.08        & 8.95    & 7.86   &  3.95 \\
Both      & 3.11    & 5.22   & 11.36       & 24.41   & 23.82       &  4.44 \\ \midrule
Cross validation & 2.78 & 1.30 & 5.48 & 6.61 & 6.00 & 3.50 \\
\bottomrule
\end{tabular}
\caption{RMSE on unseen source languages or target languages. Note that for transfer tasks, target languages refer to transfer languages.} 
\label{tab:unseen}
\end{table*}
